In Defence of Visual Analytics Systems: Replies to Critics

The last decade has witnessed many visual analytics (VA) systems that make successful applications to wide-ranging domains like urban analytics and explainable AI. However, their research rigor and contributions have been extensively challenged within the visualization community. We come in defence of VA systems by contributing two interview studies for gathering critics and responses to those criticisms. First, we interview 24 researchers to collect criticisms the review comments on their VA work. Through an iterative coding and refinement process, the interview feedback is summarized into a list of 36 common criticisms. Second, we interview 17 researchers to validate our list and collect their responses, thereby discussing implications for defending and improving the scientific values and rigor of VA systems. We highlight that the presented knowledge is deep, extensive, but also imperfect, provocative, and controversial, and thus recommend reading with an inclusive and critical eye. We hope our work can provide thoughts and foundations for conducting VA research and spark discussions to promote the research field forward more rigorously and vibrantly.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/sec5Reflection.tex <==
\section{Reflection}
We asked participants about ``the most important problem in VA research''.
From their feedback, we identified eight critical problems which have sparked considerable interest, discussions, and critical reflections.
We summarize them as follows and the interview data can be found in the supplemental material.

% From the interviews, 
% we identify eight critical problems of research on VA systems (\autoref{fig:grandproblem}),
% which have sparked considerable interest, discussions, and critical reflections.
% We summarize them as follows:

\textbf{Usability}. Four participants raised concerns on usability, \eg~``many application papers do not put into actual application because the systems are too complex to use'' (P1). To solve the problem, P15 suggested ``studying how to simplify the design and improve the usability'' and P4 advocated ``simplifying designs should become a design rationale for every VA system.''
% It could be helpful to explore systematic usability engineering methods~\cite{nielsen1994usability} to improve usability.

\textbf{Evaluation}. Ten participants mentioned the evaluation that was mainly based on case studies and expert interviews. Such methods are sometimes considered insufficient and informal. P4 who worked in the industry said, ``evaluation is a vital problem. We need more formal approaches to evaluate VA systems. In the industry, software needs to be tested. There needs more formal evaluation with end-users in real scenarios.'' P5 said, ``we need to study the standards for evaluating VA systems, standards that are both appreciated by other domains and feasible. The VAST challenge is currently exploring this problem.''

% There needs to propose and test additional methods that can be feasible and more rigorous,
% \eg~promoting a new paper type, namely deployment paper, to encourage continuing longitudinal studies for VA systems that had been published as application papers before.

\textbf{Deployment}. Five participants talked about the deployment of VA systems since only a few systems claim actual deployment.
% Many VA systems are developed in the laboratory and not deployed in the field. 
More empirical studies are needed to understand the challenges of field deployment, especially in the industry, to increase the impacts.
P6 shared an interesting viewpoint, ``deployment needs enormous resources and years. To encourage deployment, we need a new awarding mechanism. For example, we can set up a paper type, called deployment paper, which allows researchers to report insights on the deployment of already published VA systems. What are the insights learned through deployment? These can be valuable to other domains.''

\textbf{Replicability}. 
Three participants discussed replicability. They linked it with open-source, which is a common method for improving replicability.
P11 said, ``VA systems are software. If we do not open-source VA systems, other domains cannot use our tools and appreciate the values of our systems.''
However, only a few VA systems publish the programs (\eg~\cite{cheng2020dece, lange2021loon, ming2018rulematrix, strobelt2017lstmvis}).
There need more discussions and actions to promote the replicability of VA systems~\cite{fekete2020exploring}.

% Replicability has been an increasingly important principle in computer science. 
% There are many open-sourced libraries for creating data visualizations that significantly boost visualizations' influence.
% However, only a few VA systems publish the programs (\eg~\cite{cheng2020dece, lange2021loon, ming2018rulematrix, strobelt2017lstmvis}).

\textbf{Generalization}. Two concerns were regarding generalizability. P4 commented, ``VA systems are designed for a specific problem, which are hard to generalize. Can we summarize and abstract into generalizable VA techniques?''
P14 similarly asked, ``researchers are applying VA systems to different domains. Can we find general problems or tasks among different domains?''

% VA systems are often an ad-hoc solution. As a research field, it is important to study how to derive general knowledge from many ad-hoc systems, 
% \eg~by reverse-engineering VA systems to identify design (anti-)patterns and formalize ``best'' practices~\cite{canfora2011achievements}.

\textbf{Theorization}. Three participants shared their perspectives on the theoretical underpinnings of VA systems such as research methodology.
P6 commented, ``the current research on VA systems are instances of practice. With an accumulation of instances, we should summarize and improve methodological methods. For example, we should reflect on how to improve the design study methodology and how to develop and deploy VA systems?''

% The accumulation of research on VA systems creates new opportunities to reflect on existing practices.
% Such reflection can lead to refinements of methodologies,
% strengthening the theoretical underpinnings such as new taxonomies, guidelines, formalisms, conceptual models, and theoretic frameworks~\cite{chen2017pathways}.

\textbf{Intelligence}. Two participants envisioned the future of intelligent design of VA systems. For example, P14 said, ``the VA design and development procedure is currently very ad-hoc and labor-intensive. I wonder if we can summarize common patterns and automate certain steps.'' P4 echoed, ``VA systems should be more intelligent. In the industry, we hope the product to be intelligent and easy to use.''



% Designing, developing, and validating VA systems is challenging and labor-intensive. The development of AI approaches offers new potential for solving the above problems (\eg~mining design knowledge~\cite{li2021kg4vis}) and automating certain manual efforts (\eg~developing recommenders~\cite{wu2021multivision,yuan2021infocolorizer}).

\textbf{Education}. Lastly, one participant (P5) talked about the education problem, saying ``developing VA systems requires many skills such as understanding the user requirements, surveying users, developing and testing. How can we train our students?''
Those skills are broad and challenging to master.
However, there exists little educational material in training students to conduct and assess VA system research~\cite{lee2019beyond}.

% Research on VA systems requires a wide range of professional skills, 
% such as leveraging HCI approaches to understanding target users, implementing automated algorithms, and designing effective visual designs. 
% Those skills are broad and challenging to master.
% However, there exists little educational material in training students to conduct and assess VA system research~\cite{lee2019beyond}.


% 可视分析系统的开发太adhoc, 缺乏方法论的指导；可视设计的创新效果成疑，是否有效缺乏evidence；可视分析系统过于复杂，使用缺乏规范和指南，。。。，这些都是困扰领域的重大问题。AI的兴起对这些问题的解决带来一些曙光，完全可以有新的方法论来解决这些老大难问题

% 所有的committee几乎都注意到的一些共同问题：
% 1. 系统看起来非常复杂
% 2. expert interview比较ad hoc. 可视化系统的评估一直是个难题
% 3. generalization of those systems


% Interviewees proposed multiple ideas to support generalizability.
% The primary suggestion for VA systems contributors is to achieve a sufficient level of data and task abstraction.
% Such abstraction, if possible, with additional experiments could provide evidences that the VA system might apply to other similar datasets.
% Interviewees also suggested to survey existing VA systems to mine general knowledge.
% Recent research on investigating the composition patterns in multiple-view visualizations~\cite{chen2020composition} seem a promising direction.

==> sections/sec7Conclusion.tex <==
\section{Conclusion and Future Work}
Decades of research have produced a large number of VA systems.
Those VA systems are valuable and successful stories to specific application domains, yet sometimes ad-hoc.
Being ad-hoc does not mean unclear research values and rigor, however.
We must remember that Johannes Kepler's laws of planetary motion were induced from Tycho Brahe's ad-hoc observations of Mars.
We thus come in defence of VA systems by arguing the need for reflecting on existing VA system research to identify criticisms, problems, replies, and opportunities.
% Such reflection can advance the theoretical and practical underpinnings.

As one step towards this vision,
we present two interview studies with VA researchers.
Our results are a list of 36 low-level criticisms and valuable suggestions for responding to those criticisms.
Such knowledge is evidence-based and grounded but also imperfect and controversial.
We adopt a linear model to summarize and present the criticisms,
which might be insufficient.
A next step towards deeper understandings is to develop a topological model for untangling the complex network of criticisms and arguments.

Besides, our interviewees are peer researchers and thus not representative of the whole community, so is the generated knowledge.
We also plan to reach out to a broader range of interviewees, such as researchers out of our field,
industrial or governmental practitioners, and the end users of VA systems.
% We hope that our work can provide solid foundations and spark constructive discussions,
We hope that our work can provide thoughts and foundations and spark constructive discussions,
\eg~at panels, keynotes, and workshops,
to move the field forward more rigorously and vibrantly.




==> tables/abstraction.tex <==
\begin{table}[]
\small
\caption{Terminology used in problem abstraction in 30 surveyed paper in IEEE VIS 2021. Numbers in brackets indicate the counts.}
\label{table:abstraction}
\centering
\begin{tabular}{l|p{6.3cm}}
\toprule
\textbf{Class} & \textbf{Example}  \\ \hline
Task (16) & \parbox[t]{7cm}{analysis task (8) (analysis tasks, analytical tasks, analytic tasks),    \\ VA task (5) (visual analysis tasks, visualization tasks, VA task), \\ tasks (2), design tasks (1)} \\ 
Requirement (11) & design requirements (7), requirements (2), analytics requirements (1), user requirements (1) \\
Goal (9) & design goals (6), domain goals (2), overall goals (1) \\
Consideration (2) & design considerations (2) \\
Others (3) & design rationales (1), analysis factors (1), design challenges (1) \\
Workflow (2) & analysis workflow (1), three-step workflow (1) \\
\bottomrule
\end{tabular}
% \begin{tablenotes}
%   \small
%   \item **: D and V refer to the top-level sections that cover both Data and Algorithms (D) and Visual Design (V). 
% \end{tablenotes}
\end{table}





==> tables/pitfalls.tex <==
\begin{table}[!h]
\small
\caption{Summary of 38 common issues raised by reviewers. The last column (N) indicates the count.}
\label{table:pitfal}
\centering
\begin{tabular}{l|l|l|l}
\toprule
Issue & Description & Section & N \\ \hline
I-0 &  Lacking arcs of coherence and consistency & - & ? \\
I-1 &  Unclear relevance to visual analytics & Introduction & 5 \\
I-2 &  Vague/over-claimed contributions & Introduction & 6 \\
I-3 &  Relevance to the visualization community & Introduction & 3 \\
I-4 &  Missing related work & Related Work & 5 \\
I-5 &  Inadequate discussion about related work & Related Work & 1 \\
I-6 &  Unclear domain experts & Domain Problem & 7 \\
I-7 &  Lacking methodological clarity & Domain Problem & 6 \\
I-8 &  Insufficient abstraction & Domain Problem & 2 \\
I-9 &  Unclear definitions and explanations of data & Data/Algorithm & 5 \\
I-10 &  Missing technical details & Data/Algorithm & 15 \\
I-11 &  Lacking novel algorithms & Data/Algorithm & 1 \\
I-12 &  Unjustified choices of algorithms/models & Data/Algorithm & 7 \\
I-13 &  Uncertainty/stability/sensibility & Data/Algorithm & 6 \\
I-14 &  Specific technical questions & Data/Algorithm & 13 \\
I-15 &  Missing details and insufficient explanations & Visual Design & 8 \\
I-16 &  Visual design: what and why is novel? & Visual Design & 3 \\
I-17 &  Unclear rationale and insufficient justifications & Visual Design & 23 \\
I-18 &  Problematic/questionable visual designs & Visual Design & 6 \\
I-19 &  Missing justifications about alternative designs & Visual Design & 4 \\
I-20 &  Designs are over-complicated & Visual Design & 9 \\
I-21 &  Lacking an overview of workflow or system & System  & 3 \\
I-22 &  Unclear target users  & System  & 3 \\
I-23 &  Unclear novelty compared with previous work & System  & 10 \\
I-24 &  Scalability & System  & 10 \\
I-25 &  Generalizability & System  & 6 \\
I-26 &  Usability & System  & 2 \\
I-27 &  Evaluations are incomplete and insufficient & Evaluation  & 8 \\
I-28 &  Unclear evaluation protocols & Evaluation  & 9 \\
I-29 &  Lacking realism & Evaluation  & 9 \\
I-30 &  Lacking comparison with baseline approaches & Evaluation  & 8 \\
I-31 &  Lacking quantitative evaluation and feedback & Evaluation  & 5 \\
I-32 &  Insights are suspicious or not new & Evaluation  & 5 \\
I-33 &  Interpreting expert feedback  & Evaluation  & 9 \\
I-34 &  Limitations and implications & Discussion & 5 \\
I-35 &  Various presentation issues & Other & 22 \\
I-36 &  Open-source  & Other & 3 \\
I-37 &  System demonstration & Other & 3 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/secHeadings.tex <==
\begin{table*}[]
\small
\caption{Mappings between our eight-component framework to section headings in 31 surveyed papers in IEEE VIS 2021}
\label{table:secHeading}
\centering
\begin{tabular}{l|p{14cm}}
\toprule
\textbf{Ours} & \textbf{Section Headings} \\ \hline
Introduction & Introduction [31] \\
Related Work & Related work [29], Background [2], Working with hyperproperties [1], Background on bitcoin mining and mining pools [1], Background and related work [1] \\
Problem Abstraction & Background [7], Design goals [2], Design requirements [2], Methods [1], Design of coux [1], Analytic tasks [1], Task and design requirements [1], Design process and task analysis [1], Analysis factors and motivation [1], Risk-aware framework [1], Design challenges [1], Human-ai teaming for zero-shot classification [1], Tasks and workflow [1], Domain-centered design [1], Abstractions [1], Formative study [1], Informing the design [1], Design overview [1], Collaboration and domain goals [1], Biological background [1], Design methodology [1], Background and design requirements [1], User-centered design [1], Domain background [1], Development process and requirement analysis [1] \\
Data and Algorithms & Algorithm [2], Non-visual data analysis support [1], Dataset description [1], Predictive modeling [1], Data analysis [1], Data and analysis [1], Scalable neural network summarizationneurocartography [1], Data acquisition [1], Efficient dynamic clustering [1], A multilevel overview of event sequences [1], Vision based autonomous driving models [1], Geo-context aware data processing [1], Method [1], Model [1] \\
Visual Design & Visual design [3], Visualization design [2], Loon visualization design [1], Visualization and interaction [1], Vbridge [1], User interface [1], Visualization techniques [1], Design of the visualization system [1] \\
System and Implementation & Implementation [4], Overview [2], System design [2], The irvine system [1], M2 lens [1], Visual evaluation approach [1], Lumos [1], Design of visqa [1], Evis [1], Visualization system [1], Architecture [1], Visualization techniques [1], Semantic navigator [1], System implementation [1], System description [1], Coux system [1], System overview [1], Vitality [1], Visual analytics framework [1], Hypervis [1], Visual analysis of disease progression [1], Visual analytics system [1] \\
Evaluation & Evaluation [13], Case studies [4], Usage scenarios [3], User study [2], Expert evaluation [2], User evaluation [2], Example usage scenarios [2], Usage scenarios and expert review [1], Validating hypervis [1], Results [1], Experimental validation [1], Evaluation and results [1], Human experiment to evaluate neurocartography [1], Usage scenario [1], Experiments [1], Expert feedback [1], Motivating case study [1], Evaluation with domain experts [1], Use cases [1], System evaluation [1], Case study [1], Case studies and evaluation [1] \\
Discussion and Conclusion & Discussion [21], Conclusion [15], Conclusion and future work [3], Discussion and conclusion [3], Limitations [2], Discussions [2], Lessons learned and reflections [1], Conclusions [1] \\
\bottomrule
\end{tabular}
% \begin{tablenotes}
%   \small
%   \item **: D and V refer to the top-level sections that cover both Data and Algorithms (D) and Visual Design (V). 
% \end{tablenotes}
\end{table*}

